A Fast and Accurate System for Face Detection, Identification, and Verification

The availability of large annotated datasets and affordable computation power have led to impressive improvements in the performance of CNNs on various object detection and recognition benchmarks. These, along with a better understanding of deep learning methods, have also led to improved capabilities of machine understanding of faces. CNNs are able to detect faces, locate facial landmarks, estimate pose, and recognize faces in unconstrained images and videos. In this paper, we describe the details of a deep learning pipeline for unconstrained face identification and verification which achieves state-of-the-art performance on several benchmark datasets. We propose a novel face detector, Deep Pyramid Single Shot Face Detector (DPSSD), which is fast and capable of detecting faces with large scale variations (especially tiny faces). We give design details of the various modules involved in automatic face recognition: face detection, landmark localization and alignment, and face identification/verification. We provide evaluation results of the proposed face detector on challenging unconstrained face detection datasets. Then, we present experimental results for IARPA Janus Benchmarks A, B and C (IJB-A, IJB-B, IJB-C), and the Janus Challenge Set 5 (CS5).

==> other_app.tex <==
\subsection{Facial Attributes}\label{sec:face_attributes}
% Pouya
From a single face, we are able to identify facial attributes such
as gender, expression, age, skin-tone, etc. Those attributes are
very useful for applications like image retrieval, emotion
detection, and mobile security. In biometrics literature, facial
attributes are also referred to as ``soft
biometrics"~\cite{jain2004can}. Kumar \emph{et
al.}~\cite{learned2016labeled} introduced the concept of attributes
as image descriptors for face verification. They used a collection
of 65 binary attributes to describe each face image. Berg \emph{et
al.} created classfiers for each pair of people in a dataset and
then used these classifiers to create features for a face
verification classifier~\cite{learned2016labeled}. Here, rather than
manually identifying attributes, each person was described by their
likeness to other people. This is a way of automatically creating a
set of attributes without having to exhaustively hand-label
attributes on a large dataset. Recently, DCNNs have been used for
attribute classification, demonstrating impressive results. Pose
Aligned Networks for Deep Attributes (PANDA) achieved
state-of-the-art performance by combining part-based models with
deep learning to train pose-normalized DCNNs for attribute
classification~\cite{zhang2014panda}. Focusing on age and
gender,~\cite{levi2015age} applied DCNNs to the Adience dataset. Liu
\emph{et al.} used two DCNNs - one for face localization and the
other for attribute recognition - and achieved impressive results on
the CelebA and LFWA datasets, outperforming PANDA on many
attributes~\cite{liu2015deep}.

\begin{figure}[htp!]
	\centering
	\includegraphics[width=0.6\textwidth]{attribute_aa.pdf}\\
	\caption{A sample pipeline of a face attribute detection algorithm
		for mobile authentication~\cite{samangouei2016convolutional}.}
	\label{fig:face_attribute}
\end{figure}

Instead of treating each attribute to be
independent,~\cite{siddiquie2011image} exploits the correlation
amongst attributes to improve image ranking and retrieval by using
independently trained attribute classifiers and then learning
pairwise correlations based on the outputs of these classifiers.
Hand~\emph{et al.}~\cite{hand2017attribute} train a single attribute network which classifies 40
attributes, sharing information throughout the network, and by
learning the relationships among all the 40 attributes, not just
attribute pairs. Ranjan~\emph{et al.}~\cite{ranjan2016all} train a
single deep network with multi-task learning which can
simultaneously perform face detection, facial landmark detection,
face recognition, 3D head pose estimation, gender classification,
age estimation, and smile detection. Recently, Gunther~\emph{et al.} proposed the AFFACT~\cite{gunther2016affact} algorithm that performs alignment-free facial attribute classification. It uses a data augmentation technique that  allows a network to classify facial attributes without requiring alignment beyond detected face bounding boxes. The algorithm achieves state-of-the-art results on CelebA~\cite{liu2015deep} dataset with an ensemble of three networks.

In addition, some of the facial attributes can be
used~\cite{parkhi_deep_2015} to boost the mobile authentication
performance. The recent method of Attribute-based Continuous
Authentication (ACA)
~\cite{samangouei2015attribute,samangouei2017facial} shows that
large number of attributes by themselves can give good authentication results on mobile phones. They are semantic features which are
easier to learn than facial identities. Also, if they are learned on
facial parts, they become less complex. By leveraging these two
qualities, Samangouei \emph{et.
al.}~\cite{samangouei2016convolutional} designed efficient DCNN
architectures suitable for mobile devices. The pipeline in
Figure~\ref{fig:face_attribute} illustrates how facial attributes
are used for mobile authentication.
%The overview of our method is presented in Figure 1.

